Contrastive Object Detection Using Knowledge Graph Embeddings

Object recognition for the most part has been approached as a one-hot problem that treats classes to be discrete and unrelated. Each image region has to be assigned to one member of a set of objects, including a background class, disregarding any similarities in the object types. In this work, we compare the error statistics of the class embeddings learned from a one-hot approach with semantically structured embeddings from natural language processing or knowledge graphs that are widely applied in open world object detection. Extensive experimental results on multiple knowledge-embeddings as well as distance metrics indicate that knowledge-based class representations result in more semantically grounded misclassifications while performing on par compared to one-hot methods on the challenging COCO and Cityscapes object detection benchmarks. We generalize our findings to multiple object detection architectures by proposing a knowledge-embedded design for keypoint-based and transformer-based object detection architectures.

==> tables/coco_val_confusions.tex <==
\begin{table}
\footnotesize
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lll}
\toprule
GT         & \multicolumn{3}{c}{Predictions} \\
           & Faster R-CNN                                                                               & CenterNet                                                                                  & Faster R-CNN GloVe                                                                      \\ \midrule
Person     & \begin{tabular}[c]{@{}l@{}}Dog: 0.16\\ Chair: 0.10 \\ Cat: 0.06 \\\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Handbag: 0.19 \\ \ Surfboard: 0.06 \\ Dog: 0.04 \end{tabular}   & \begin{tabular}[c]{@{}l@{}} Bicycle: 0.92\\ Dog: 0.06 \\ Motorcycle: 0.01 \end{tabular} \\ \midrule
Motorcycle & \begin{tabular}[c]{@{}l@{}}Bicycle: 0.44 \\ Person: 0.13 \\ Backpack: 0.03 \end{tabular}   & \begin{tabular}[c]{@{}l@{}}Bicycle: 0.34\\ Person: 0.28 \\ Bench: 0.10 \end{tabular}       & \begin{tabular}[c]{@{}l@{}}Bicycle: 0.67\\ Car: 0.24 \\ Bus: 0.19 \end{tabular}         \\ \midrule
Pizza      & \begin{tabular}[c]{@{}l@{}}Sandwich: 0.43 \\ Dining table: 0.22 \\ Bowl: 0.08\end{tabular} & \begin{tabular}[c]{@{}l@{}}Sandwich: 0.27\\ Dining table: 0.22 \\ Oven: 0.07 \end{tabular} & \begin{tabular}[c]{@{}l@{}}Sandwich: 0.66 \\ Cake: 0.23 \\ Broccoli: 0.07 \end{tabular} \\
\bottomrule
\end{tabular}
}
\caption{Top 3 relative false positive counts for person, motorcycle, and pizza classes on COCO 2017 validation dataset. The predicted bounding boxes were assigned to the ground truth boxes by an IoU threshold, allowing many-to-one matching.}
\label{tab:coco_confusions}
	\vspace{-0.2cm}
\end{table}

==> tables/results_ablation.tex <==
\begin{table*}
\footnotesize
\centering
\begin{tabular}{lll|ccc|ccc}
\toprule
{Model}           & {Object Class Representation} & {Embedding Loss} & \multicolumn{3}{c|}{{COCO 2017 Val}} & \multicolumn{3}{c}{{Cityscapes Val}} \\
\cmidrule{4-9}
                                 &                                              &                                 & AP       & $\mathbf{AP_{50}}$    & $\mathbf{AP_{75}}$    & $\mathbf{AP}$       & $\mathbf{AP_{50}}$    & $\mathbf{AP_{75}}$    \\
                                 \midrule
\multirow{6}{*}{Faster RCNN-FPN} & GloVe                                        & TransR                          & 40.4     & 61.7       & \textbf{45.2}       & 41.7     & 64.9       & 44.3       \\
                                 & GloVe                                        & DistMult                        & \textbf{41.7}     & \textbf{62.3}       & 43.9       & \textbf{43.6}     & \textbf{66.9}       & \textbf{45.7}       \\
                                 & ConceptNet                                   & TransR                          & 40.2     & 61.0         & 43.8       & 40.6     & 66.5       & 43.5       \\
                                 & ConceptNet                                   & DistMult                        & 41.0       & 62.2       & 44.5       & 42.4     & 66.4       & 45.1       \\
                                 & COCO 2017 train co-occurrences               & TransR                          & 38.6     & 60.9       & 42.1       & 40.4     & 65.9       & 43.4       \\
                                 & COCO 2017 train co-occurrences               & DistMult                        & 40.1     & 59.5       & 41.0       & 39.5     & 63.4       & 42.9       \\
                                 \midrule
\multirow{6}{*}{CenterNet}       & GloVe                                        & TransR                          & 27.0     & 48.4       & 30.8       & 27.6     & 52.6       & 30.8       \\
                                 & GloVe                                        & DistMult                        &          &            &            &          &            &            \\
                                 & ConceptNet                                   & TransR                          & 26.2     & 50.8       & 32.4       & 27.8     & 51.7       & 33.4       \\
                                 & ConceptNet                                   & DistMult                        &          &            &            &          &            &            \\
                                 & COCO 2017 train co-occurrences               & TransR                          &          &            &            &          &            &            \\
                                 & COCO 2017 train co-occurrences               & DistMult                        &          &            &            &          &            &            \\
                                 \midrule
\multirow{6}{*}{DETR}            & GloVe                                        & TransR                          &          &            &            &          &            &            \\
                                 & GloVe                                        & DistMult                        &          &            &            &          &            &            \\
                                 & ConceptNet                                   & TransR                          &          &            &            &          &            &            \\
                                 & ConceptNet                                   & DistMult                        &          &            &            &          &            &            \\
                                 & COCO 2017 train co-occurrences               & TransR                          &          &            &            &          &            &            \\
                                 & COCO 2017 train co-occurrences               & DistMult                        &          &            &            &          &            &            \\
                                 \bottomrule
\end{tabular}%
\caption{Ablation study over prediction head configurations.
The validation set results over regression target vectors derived from varying knowledge sources.
The top section shows baseline results in Detectron2 with standard one-hot classification heads.
The center section shows results on the COCO validation set, and the left section shows results on the cityscapes dataset. 
Ablation is performed over proposed regression heads, that vary in the type of target vectors representing object types, and whether or not a message passing through the scene graph structure was used.}
\label{tab:results_ablation}
\end{table*}
